Federated Contrastive Learning of Graph-Level Representations

Graph-level representations (and clustering/classification based on these representations) are required in a variety of applications. Examples include identifying malicious network traffic, prediction of protein properties, and many others. Often, data has to stay in isolated local systems (i.e., cannot be centrally shared for analysis) due to a variety of considerations like privacy concerns, lack of trust between the parties, regulations, or simply because the data is too large to be shared sufficiently quickly. This points to the need for federated learning for graph-level representations, a topic that has not been explored much, especially in an unsupervised setting. Addressing this problem, this paper presents a new framework we refer to as Federated Contrastive Learning of Graph-level Representations (FCLG). As the name suggests, our approach builds on contrastive learning. However, what is unique is that we apply contrastive learning at two levels. The first application is for local unsupervised learning of graph representations. The second level is to address the challenge associated with data distribution variation (i.e. the ``Non-IID issue") when combining local models. Through extensive experiments on the downstream task of graph-level clustering, we demonstrate FCLG outperforms baselines (which apply existing federated methods on existing graph-level clustering methods) with significant margins.

==> input/back_up_info.tex <==


\section{Analysis}
\label{sec: analysis}



% \subsection{Additional Experiments}

% \subsubsection{\textbf{Centralized version of different CL models}}



\subsection{Potential theoretical basis, FL+CL}

Analysis track: inspired by ensemble distillation for model fusion~\cite{lin2020ensemble}. The current FCLG can be generalized as a special case of the ensembling techniques. 

   \begin{enumerate}
       \item FCLG: server assigned one model to each client with the same initialization, Utilize instance-level contrastive learning (inner and across clients). 
       \item More general case, K model (with same initialization) on the server, send out to each client and pull back parameters after local updates. Now on server with a collection of unlabelled data and doing ensembling (knowledge distillation) for model fusion. 
       \item When explaining model fusion, may Use elegant Bayesian interpretation of ensemble methods~\cite{shi2021_fed}.
       \item Significance: try to build connection between the two steps: 1) local drift prevention 2) model aggregation. Unify both as ensembling techniques.
   \end{enumerate}
   
% \subsection{Extension tasks}   

% \begin{enumerate}
%     % \item Ensemble technique~\cite{lin2020_ensemble_distillation,laine2016_temporal,shi2021_fed}. Potential relation to the ensemble distillation for model fusion.
%     % \item Extension task: personalized model on each model through knowledge distillation.
%     \item On top of general model, form personalized model on each client.
%     % \item Investigate supervised graph classification for FCLG.
% \end{enumerate}


\subsection{Current Progress}

\begin{enumerate}
    \item Implemented a loosen and more interpretable version of the algorithm. The server will conduct intra-contrast its own dataset to improve the generalization performance.
    \item Main ideal of this algorithm: remove the original inter-contrast step, instead the server will get its own share of data and perform its own contrastive learning. Here allowing a separate central server dataset have been used in other Fed-Ensembling works like ~\cite{lin2020ensemble,chen_2020_fedbe}. 
    \item This vanilla version of the model can be further modified to include more ensembling techniques and can possibly have more backbones from ensembling analysis and knowledge distillation~\cite{chen_2020_fedbe}.
\end{enumerate}





\subsection{Thinking Notes}

Why the local drift in clients can damage the generalization performance? A very possible reason will be that intra-contrasting lose sight of other data samples from other clients.  



\begin{algorithm}[tbh]
	\caption{Vanilla Ensembling on Contrastive Learning} 
	\label{alg:FCLG generalized}
	\begin{itemize}
    	\Statex{\textbf{Input}: local training epochs $E$, communication rounds $T$, number of clients $K$
    	}
    	\Statex{\textbf{Output}: learned model parameters $\omega^{T}$ }
	\end{itemize}
	\begin{algorithmic}[1]
	\State{\textbf{Server:}}
	\State{initialize $\omega^{0}$}
	\For{$j = 0, 1, \cdots, T-1 $} 
	    \For{$ i = 1, 2, \cdots, K$ in parallel}
	        \State{send global model $\omega^{j}$ to $C_{i}$}
	        \State{$\omega_{i}^{j} \gets $ \textbf{Client($i, \omega^{j}$)}}
	    \EndFor
	    \State{$\omega^{j+1} \gets \sum^{K}_{i}\frac{|S^{i}|}{|S|}\omega^{j}_{i}$}
        \For{each batch of graphs $ G_{b} \in S_{0}$}
         \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
            \State{$U^{t} \gets g(f_{\omega^{t}_{i}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}_{i}}(G_{d}) )$}
            \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} }
            \State{SGD update on $\omega^{t}_{i}$}
    	\EndFor
	\EndFor
	\State{return $\omega^{T}$}
	%% =============Sever above =================
	\State{\textbf{Client($i, \omega^{j}$):}}
    \State{$\omega^{0}_{i} \gets \omega^{j}$}
    \For{$t = 1, 2, \cdots, E $} 
        \For{each batch of graphs $ G_{b} \in S^{i}$}
         \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
            % \State{$H_{c}^{t} \gets f_{\omega^{t}_{i}}(G_{b})$; $\widehat{H}_{c}^{t} \gets f_{\omega^{t}_{i}}(G_{d})$}
            \State{$U^{t} \gets g(f_{\omega^{t}_{i}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}_{i}}(G_{d}) )$}
            % \State{ $U_{s} \gets g(f_{\omega^{j}}(G_{b})) $; $U_{c}^{t-1} \gets g(f_{\omega_{i}^{t-1}}(G_{b})) $}
            \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} }
            % \State{$l_{tot} \gets l_{inter} +  l_{intra} $ }  % 
            \State{SGD update on $\omega^{t}_{i}$}
    	\EndFor
	\EndFor
	\State{return $\omega^{E}_{i}, U^{E}_{i}$ }
	\end{algorithmic} 
\end{algorithm}   



\begin{theorem}[Domain adaptation \cite{ben2010theory}] \label{thm:simplified_adaptation_empirical_bound}
	Considering the distributions $\mathcal{D}_S$ and $\mathcal{D}_T$,
	for every $h \in \mathcal{H}$ and any $\delta \in (0, 1)$,
	with probability at least $1 - \delta$ (over the choice of the samples),
	there exists:
	\begin{align}
		\textstyle
		L_{\mathcal{D}_T}(h)
		\leq L_{\mathcal{D}_S}(h) + \frac{1}{2} d_{\mathcal{H} \Delta \mathcal{H}} (\mathcal{D}_S, \mathcal{D}_T) + \lambda \,,
	\end{align}
	where $\lambda = L_{\mathcal{D}_S}(h^\star) + L_{\mathcal{D}_T}(h^\star)$.
	$h^\star := \argmin_{h \in \mathcal{H}} L_{\mathcal{D}_S} (h) + L_{\mathcal{D}_T} (h) $
	corresponds to \emph{ideal joint hypothesis} that minimizes the combined error.
\end{theorem}



\begin{table*}[tbh]
    \small
    \centering
    \caption{FCLG ensemble vanilla model graph-level clustering performance for Non-IID client data. Graph data are split into 6 parts with specific skewed distribution and respective EMD values provided alongside each dataset name. Metric results (\%) are generated from 10 runs of experiments with converged values after specific communication rounds.
}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{llrrrrr}
    \hline
    Model & Metric & PROTEINS (0.5774) & ENZYMES (1.2667) & DHFR (0.5694) & NCI1 (0.5995) \\
    \hline
    FCLG vanilla
    & Accuracy  &  $ 64.60 \pm 1.31 $ & $ 30.50 \pm 0.00 $  & $ 60.01 \pm 0.06 $  &  $ 61.10 \pm 0.40 $ \\
    & F1-macro  &  $ 64.48 \pm 1.24 $  & $ 30.36 \pm 0.00 $ &  $ 55.86 \pm 0.08 $ &  $ 57.52 \pm 0.59 $  \\
    \hline
    \end{tabular} 
    \end{adjustbox}
    % }
    \label{tab: Ensemble Non-IID graph-level clustering}
\end{table*}


% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figure/tmp/semi_unsup/DHFR_Classify_val_metric_epoch.pdf}
%          \caption{DHFR}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figure/tmp/semi_unsup/Enzymes_Classify_val_metric_epoch.pdf}
%          \caption{ENZYMES}
%      \end{subfigure}
%      fill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figure/tmp/semi_unsup/NCI1_Classify_val_metric_epoch.pdf}
%          \caption{NCI1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figure/tmp/semi_unsup/Protein_Classify_val_metric_epoch.pdf}
%          \caption{Protein}
%      \end{subfigure}
%     \caption{FCLG semi-supervised graph classification training process}
%     \label{fig: FCLG semi-supervised graph classification}
% \end{figure*} 



% \begin{algorithm}[tbh]
% 	\caption{Embedding sharing contrasting} 
% 	\label{alg:FCLG emb share}
% 	\begin{itemize}
%     	\Statex{\textbf{Input}: local training epochs $E$, communication rounds $T$, number of clients $K$
%     	}
%     	\Statex{\textbf{Output}: learned model parameters $\omega^{T}$ }
% 	\end{itemize}
% 	\begin{algorithmic}[1]
% 	\State{\textbf{Server:}}
% 	\State{initialize $\omega^{0}$}
% 	\For{$j = 0, 1, \cdots, T-1 $} 
% 	    \For{$ i = 1, 2, \cdots, K$ in parallel}
% 	        \State{send global model $\omega^{j}$ to $C_{i}$}
% 	        \State{$U^{j}_{i} \gets $ \textbf{Client($i, \omega^{j}$)}}
% 	    \EndFor
% 	    \State{Perform inter-contrast in between $\{U^{j}\}$}. 
% 	   % Or other ensambling techs among clients. 
% 	   % \State{$\omega^{j+1} \gets \sum^{K}_{i}\frac{|S^{i}|}{|S|}\omega^{j}_{i}$}
% 	\EndFor
% 	\State{return $\omega^{T}$}
% 	%% =============Sever above =================
% 	\State{\textbf{Client($i, \omega^{j}$):}}
%     \State{$\omega^{0}_{i} \gets \omega^{j}$}
%     \For{$t = 1, 2, \cdots, E $} 
%         \For{each batch of graphs $ G_{b} \in S^{i}$}
%          \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
%             % \State{$H_{c}^{t} \gets f_{\omega^{t}_{i}}(G_{b})$; $\widehat{H}_{c}^{t} \gets f_{\omega^{t}_{i}}(G_{d})$}
%             \State{$U^{t} \gets g(f_{\omega^{t}_{i}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}_{i}}(G_{d}) )$}
%             % \State{ $U_{s} \gets g(f_{\omega^{j}}(G_{b})) $; $U_{c}^{t-1} \gets g(f_{\omega_{i}^{t-1}}(G_{b})) $}
%             \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} }
%             % \State{$l_{tot} \gets l_{inter} +  l_{intra} $ }  % 
%             \State{SGD update on $\omega^{t}_{i}$}
%     	\EndFor
% 	\EndFor
% 	\State{return $\omega^{E}_{i}, U^{E}_{i}$ }
% 	\end{algorithmic} 
% \end{algorithm}   



\subsection{A Bayesian perspective}
FedBE~\cite{chen_2020_fedbe} proposed to view the problem of model drift from a Bayesian perspective. In Bayesian learning, it is the posterior distribution $p(w|\mathcal{D})$ of the global model being learned, from which $\bar{w}$ and $w^\star$ can be regarded as two particular samples (point estimates). 
Denote by $p(y |x; w)$ the output probability of a global model $w$,
one approach to mitigate model drift is to perform Bayesian inference \citep{neal2012bayesian,barber2012bayesian} for prediction, integrating the outputs of all possible models w.r.t. the posterior

\begin{align}
p(y |x; \mathcal{D}) = \int  p(y |x; w) p(w|\mathcal{D}) dw \label{eq_Bayesian}
\end{align}


rather than relying on a single point estimate. While the equation above is intractable in general, we can approximate it by the Monte Carlo method, sampling $M$ models for model ensemble

\textbf{Bayesian model ensemble: } 

\begin{align}
p(y |x; \mathcal{D}) \approx \frac{1}{M}\sum_{m=1}^M p(y |x; w^{(m)}), \text{ where } w^{(m)}\sim p(w|\mathcal{D}). \label{eq_MC}
\end{align}


\subsection{Bayesian model ensemble with approximated posteriors}
\label{ss_BME}

how to estimate $p(w|\mathcal{D})$ in federated learning, given merely client models $\{w_i\}$?

FedBE~\cite{chen_2020_fedbe} resorted to a recently proposed idea, named stochastic weight average-Gaussian (SWAG)~\citep{maddox2019simple}, for estimating the posterior. 
swag employed a cyclical or constant learning rate in SGD, following SWA~\citep{izmailov2018averaging}. swag then constructs a Gaussian distribution $p(w|\mathcal{D})$ by fitting the parameters to the model weights it traverses in SGD. 

% In federated learning, by rewriting $w_i$ as $\bar{w} - g_i$, where $g_i = -(w_i - \bar{w})$ denotes the $K$-step stochastic gradient on a mini-batch $\mathcal{D}_i\subset\mathcal{D}$ \citep{mcmahan2017communication}, we can indeed view each client's model $w_i$ as taking $K$-step \SGD to traverse the weight space of global models.

% \paragraph{Gaussian.} To this end, we propose to fit a diagonal Gaussian distribution $\mathcal{N}(mu, \Sigma_\text{diag})$ to the clients' models $\{w_i\}$  following~\citep{maddox2019simple},
% \begin{align}
% mu = \sum_i \frac{|\mathcal{D}_i|}{|\mathcal{D}|}w_i, \hspace{20pt}\Sigma_\text{diag} =  \text{diag}\left(\sum_i \frac{|\mathcal{D}_i|}{|\mathcal{D}|}(w_i - mu)^2\right), \label{eq_Gaussian}
% \end{align}
% from which we can sample $\{w^{(m)}~\sim\mathcal{N}(mu, \Sigma_\text{diag})\}_{m=1}^M$ for model ensemble (cf. \autoref{eq_MC}). Here $(\cdot)^2$ means taking element-wise square. We note that, both the clients' models $\{w_i\}$ and \FedAvg $\bar{w}$ are possible samples from $\mathcal{N}(mu, \Sigma_\text{diag})$.


\paragraph{SWA for knowledge distillation.} Optimizing $w$ using standard SGD, however, may arrive at a suboptimal solution: the resulting $w$ can have much worse test accuracy than ensemble.
We identify one major reason: the ensemble prediction $\hat{p}_j$ can be noisy ($\argmax_c \hat{p}_j[c]$ is not the true label of $x_j$), especially in the early rounds of FL. The student model $w$ thus may over-fit the noise. 
% We note that, this finding does not contradict our observations in~\autoref{ss_BME}: Bayesian model ensemble has higher test accuracy than \FedAvg but is still far from being perfect (\ie, $100\%$ accuracy). 
% To address this issue, we apply SWA~\citep{izmailov2018averaging} to train $w$. SWA employs a cyclical learning rate schedule in SGD by periodically imposing a sharp increase in step sizes and averages the weights of models it traverses, enabling $w$ to jump out of noisy local minimums.

==> input/comments.tex <==
\clearpage
% \appendix
\onecolumn

\section{Editing Plan}

\subsection{Limitations in Chapter6}

Following contents will be added to the end of Chpater6 as limitations

\begin{enumerate}
    \item The vulnerability of Federated Learning in privacy protection. Additional procedures will be needed like encoding the model parameters, which is covered in another track of research in federated learning.
    \item The lack of theoretical support on the inter-contrast mechanism. 
\end{enumerate}


\subsection{Centralized training}

In this condition, we have all data available in the central server. Hence, we perform intra-contrast among all graphs, yielding Intra-central. However, this method only has one-level of contrasting mechanism and hence will have poorer learning power than FCLG.

\textbf{\textcolor{red}{Question}}:
Shall we implement another version of centralized training and how?


\begin{table*}[tbh]
    \small
    \centering
    \caption{Including the centralized training, FCLG graph-level clustering performance for Non-IID client data. Graph data are split into 6 clients with specific skewed distribution and respective EMD values provided alongside each dataset name. Metric results (\%) are generated from 10 runs of experiments with converged values after specific communication rounds.
}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{llrrrrr}
    \hline
    Model & Metric & PROTEINS (0.5774) & ENZYMES (1.2667) & DHFR (0.5694) & NCI1 (0.5995) \\
    \hline
    InfoGraph-FedAvg & Accuracy  & $ 62.40 \pm 1.59 $ & $ 26.00 \pm 1.23 $  & $ 56.59 \pm 0.05 $  & $ 57.82 \pm 0.19 $  \\
    & F1-macro  & $ 61.58 \pm 1.19 $  & $ 25.85 \pm 1.34 $ & $ 55.51 \pm 0.05 $ & $ 57.59 \pm 0.20 $ \\
    \hline
    InfoGraph-FedProx & Accuracy  & $ 60.97 \pm 2.39 $  & $ 27.93 \pm 0.15 $  & $ 57.54 \pm 0.00 $  & $ 59.15 \pm 0.56 $ \\
    & F1-macro  & $ 60.47 \pm 2.19 $  & $ 27.89 \pm 0.18 $ & $ 57.35 \pm 0.00 $ & $ 58.85 \pm 0.85 $  \\
    \hline
    MVGRL-FedAvg & Accuracy  & $ 59.35 \pm 0.10 $  & $ 17.33 \pm 0.00 $  & $ 61.11 \pm 0.00 $  & $ 50.07 \pm 0.00 $  \\
    & F1-macro  & $ 37.25 \pm 0.04 $ & $ 6.12 \pm 0.00 $ & $ 38.25 \pm 0.00 $ & $ 33.41 \pm 0.00 $  \\
    \hline
    MVGRL-FedProx  & Accuracy  & $ 59.30 \pm 0.20 $ & $ 17.50 \pm 0.00 $  & $ 61.11 \pm 0.00 $  & $ 50.07 \pm 0.00 $  \\
    & F1-macro  & $ 37.22 \pm 0.08 $  & $ 6.45 \pm 0.00 $ & $ 38.25 \pm 0.00 $ & $ 33.41 \pm 0.00 $  \\
    \hline
    \hline
    FCLG 
    & Accuracy  &  $ 69.90 \pm 2.59 $ & $ 32.45 \pm 0.45 $  & $ 67.01 \pm 0.83 $  &  $ 61.42 \pm 0.07 $ \\
    & F1-macro  &  $ 69.12 \pm 1.97 $  & $ 30.61 \pm 0.40 $ &  $ 66.59 \pm 0.76 $ &  $ 60.03 \pm 0.07 $  \\
    \hline
    FCLG-H
    & Accuracy  & $ 69.95 \pm 2.57 $  & $ 32.03 \pm 1.22 $  & $ 65.38 \pm 0.84 $  &  $ 61.45 \pm 0.06 $  \\
    & F1-macro  & $ 68.98 \pm 2.08 $  & $ 29.76 \pm 1.53 $ & $ 64.93 \pm 0.90 $ & $ 60.05 \pm 0.07 $  \\
    \hline
    Intra-FedAvg 
    & Accuracy  & $ 70.41 \pm 2.35 $  & $ 30.50 \pm 0.07 $  &  $ 60.22 \pm 1.19 $  & $ 61.55 \pm 0.10 $  \\
    & F1-macro  &  $ 69.29 \pm 1.93 $ &  $ 29.96 \pm 0.07 $ &  $ 59.43 \pm 1.18 $ & $ 60.23 \pm 0.10 $ \\
    \hline
    % Intra-H-FedAvg
    % & Accuracy  & $ 70.39 \pm 1.86 $ & $ 30.48 \pm 0.05 $  & $ 60.05 \pm 0.90 $  & $ 61.79 \pm 0.11 $ \\
    % & F1-macro  &  $ 69.23 \pm 1.49 $  & $ 29.93 \pm 0.03 $ &  $ 58.92 \pm 1.07 $ &  $ 60.36 \pm 0.13 $  \\
    % \hline
    Intra-KL 
    & Accuracy  &  $ 66.58 \pm 1.14 $ & $ 31.00 \pm 0.00 $  & $ 61.44 \pm 0.25 $  &  $ 61.31 \pm 0.14 $ \\
    & F1-macro  &  $ 66.07 \pm 0.99 $  & $ 29.95 \pm 0.00 $ &  $ 58.59 \pm 0.24 $ &  $ 59.95 \pm 0.17 $  \\
    \hline
    Intra-MSE
    & Accuracy  &  $ 64.80 \pm 2.17 $ & $ 29.83 \pm 0.99 $  & $ 61.48 \pm 0.05 $  &  $ 61.52 \pm 0.07 $ \\
    & F1-macro  &  $ 64.72 \pm 2.09 $  & $ 29.24 \pm 1.19 $ &  $ 59.70 \pm 0.04 $ &  $ 60.25 \pm 0.08 $  \\
    \hline
    \hline
    Intra-central
    & Accuracy  & $ 66.81 \pm 0.11 $  & $ 27.80 \pm 0.78 $  & $ 58.42 \pm 0.96 $  & $ 58.41 \pm 0.20 $  \\
    & F1-macro  & $ 64.87 \pm 0.10 $  & $ 27.55 \pm 0.69 $ & $ 57.08 \pm 4.22 $ & $ 58.32 \pm 0.19 $ \\
    \hline
    \end{tabular} 
    \end{adjustbox}
    % }
    \label{tab: Non-IID graph-level clustering with central}
\end{table*}



Below we compare the centralize training algorithms and the FCLG algorithm.


\begin{algorithm}[tbh]
	\caption{Intra-central for graph-level representations} 
	\label{alg:Intra-central Train}
	\begin{itemize}
    	\Statex{\textbf{Input}: union of all graphs data $S$, training epochs $E$.}
    	\Statex{\textbf{Output}: learned model parameters $\omega^{E}$ }
	\end{itemize}
	\begin{algorithmic}[1]
    \For{$t = 1, 2, \cdots, E $} 
        \For{each batch of graphs $ G_{b} \in S$}
         \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
            \State{$U^{t} \gets g(f_{\omega^{t}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}}(G_{d}) )$}
            \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} }
            \State{SGD update on $\omega^{t}$}
    	\EndFor
	\EndFor
	\State{return $\omega^{E}$}
	\end{algorithmic} 
\end{algorithm}


\begin{algorithm}[tbh]
	\caption{FCLG training for graph-level representations} 
	\label{alg:FCLG Train comments}
	\begin{itemize}
    	\Statex{\textbf{Input}: local training epochs $E$, communication rounds $T$, number of clients $K$ and $\gamma$ the fraction of clients participating in each round.
    	}
    	\Statex{\textbf{Output}: learned model parameters $\omega^{T}$ }
	\end{itemize}
	\begin{algorithmic}[1]
	\State{\textbf{Server:}}
	\State{initialize $\omega^{0}$}
	\For{$j = 0, 1, \cdots, T-1 $} 
            \State{Randomly sample a subset of $K_{\gamma}$ clients}
	    \For{$ i = 1, 2, \cdots, K_{\gamma}$ in parallel}
	        \State{send global model $\omega^{j}$ to $C_{i}$}
	        \State{$\omega_{i}^{j} \gets $ \textbf{Client($i, \omega^{j}$)}}
	    \EndFor
	    \State{$\omega^{j+1} \gets \sum^{K_{\gamma}}_{i}\frac{|S^{i}|}{|S|}\omega^{j}_{i}$}
	\EndFor
	\State{return $\omega^{T}$}
	%% =============Sever above =================
	\State{\textbf{Client($i, \omega^{j}$):}}
    \State{$\omega^{0}_{i} \gets \omega^{j}$}
    \For{$t = 1, 2, \cdots, E $} 
        \For{each batch of graphs $ G_{b} \in S^{i}$}
         \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
            % \State{$H_{c}^{t} \gets f_{\omega^{t}_{i}}(G_{b})$; $\widehat{H}_{c}^{t} \gets f_{\omega^{t}_{i}}(G_{d})$}
            \State{$U^{t} \gets g(f_{\omega^{t}_{i}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}_{i}}(G_{d}) )$}
            \State{ $U_{s} \gets g(f_{\omega^{j}}(G_{b})) $; $U_{c}^{t-1} \gets g(f_{\omega_{i}^{t-1}}(G_{b})) $}
            \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} and $l_{inter}$ from Eq.\ref{eq: graph-level CL server and client}}
            \State{$l_{tot} \gets l_{inter} +  l_{intra} $ }  % 
            \State{SGD update on $\omega^{t}_{i}$}
    	\EndFor
	\EndFor
	\State{return $\omega^{E}_{i}$}
	\end{algorithmic} 
\end{algorithm}

==> input/reviews.tex <==
\newpage
\onecolumn

\section{Reviews}

We thank all reviewers for insightful and detailed reviews. The responses to the points raised are included below.


Reviewer-1:

Q1: Federated learning is distributed by definition. However, this aspect is not clearly articulated in the paper. 
A1: We explicitly introduced Federated Learning as a distributed computing technique. For example, in section I (Introduction) 2nd paragraph “federated learning involves training centralized models, while the data remains decentralized…”. Similar descriptions can be found in the corresponding part in Section II. In section IV, we split training data into multiple clients and compare results based on the data distribution (IID or Non-IID).

Q2: Can this work be extended to subgraph-level learning? How about node-level representation learning (when on graph is distributed across different nodes)?
A2: Our method focuses on graph-level representation learning only. Part of the algorithm (contrastive learning) can potentially be extended to node-level, however, algorithms have to be adjusted accordingly and performance may not be guaranteed. Subgraph level or node-level has its major concern (e.g., information loss due to decentralized storage of graph nodes and missing edges) and is out of the scope of the current work.

Reviewer-2:

Reply to the comments:
C1: In my understanding… confused about some of the comparisons.
A1: Details about the baseline construction are covered in the “Experimental Settings” part within section IV. In summary, InfoGraph and MVGRL are existing unsupervised graph-level representation methods while FedProx and FedAvg are two Federated learning schemes. We created federated unsupervised graph-level representation baselines by cross-product combination. 

C2: III.A is poorly structured… $G$ and $X$ to allow federated learning which are never stated exactly.
A2: In Section III.A, at the beginning of 3rd paragraph, $\omega$ is defined in the same sentence as its first appearance. $\omega$ means the to-be-trained machine learning model parameter set, we could further modify our text to make it clearer. $\omega_g$ means the global machine learning model parameter set to be learned through federated learning. A predefined distribution of $G$ and $X$ is given in experimental settings in Section IV (Non-IID or IID).

C3:  Functions $f_c$ and $f_s$ are undefined… till then the paper is unreadable.
A3: Functions $f_c$ and $f_s$ are defined in 2nd paragraph in III.B, they represent corresponding models (local or global) correspondingly. $x_i$ is the graph representation including both node features and graph topology for i-th graph sample. These symbols aim to simplify the mathematical expression and we will make it clearer in revision.

C4: What is equation (4) optimized for? and where is it used?
A4: Eq.4 is inter-contrasting training loss, the explanation is right below Eq.4. It is further re-written in a more concrete form in Eq. 7. 

C5: The text in section D should come much earlier in the paper.
A5: Thanks. We will reorganize it to ease reading.

C6: What do you mean by "graph-level representations U" in page 4?
A6: Yes, you are right. U = $f_c$(x; $\omega$). We will put III.D ahead of III.C to make it clear.

C7: In $l_{inter}$ we use $H_s$ Are these computed using the "frozen" incoming $\omega^j$?
A7: Yes. 

C8: InfoGraph and MVGRL are poorly described in the paper as well as the "Baselines" section that is critical for the evaluation.
A8: We would add more descriptions about these methods.

C9: It is unclear what FedProx does
A9: We could provide more descriptions about FedProx.

Questions:

Q1: In Figure 2, why isn't FCLG not compared with GIN-FedAvg and GIN-FedProx?
A1: GIN is a graph convolutional network proposed for supervised learning with advanced performance on graph-level representation learning. Hence neither GIN-FedAvg nor GIN-FedProx can handle unsupervised learning cases which are the focus of this paper. That is why contrastive learning mechanisms serve as a key part of our method. GIN, as part of neural network design, is also used in one baseline model “InfoGraph” in Table III and Table IV. 

Q2: Given the small datasets how do you split them to IID and non-ID?
A2: Data splitting is based on the graph labels distribution. To simplify the illustration, suppose we have 3 clients and there are a total of 3 labels of graphs (A, B, C). For IID we evenly split each group of graphs sharing the same labels into clients, then each client will have A/3+B/3+C/3 yielding the same distribution across clients. For Non-IID, we choose one label as the dominant for each client and rotate the dominant label, the resulting distribution on all 3 clients can be like this: 2/3A+1/6B+1/6C; 1/6A+2/3B+1/6C; 1/6A+1/6B+2/3C. The dominant fraction is controlled as a hyper-parameter depending on the degree of Non-IID.

Reviewer-3:

Q1: Alg. 1 and Fig. 1 summarize this representation…compared to a non-federated distributed method?
A1: We introduce the motivation of federated learning in Section I (Introduction) second paragraph. The scenario is data sharing can be prohibited due to privacy concerns. Non-federated cases (out of the scope of this paper) won’t induce communication costs.
Q2:  It will be nice to summarize the main ideas in the current submission.
A2: The main contributions are summarized towards the end of Section I (Introduction).

Q3: The empirical evaluation can be considerably improved…that truly requires unsupervised federated learning.
A3: We are using the datasets from TUDatasets [1] following previous graph-level federated learning works [2].

[1] TUDatasets, https://chrsmrrs.github.io/datasets/
[2] Xie, H. et al, Federated graph classification over non-iid graphs, NeuIPS, 2021

Reviewer-4:

Q1: Concerning scalability, it would… in papers with FL settings and related works.
A1: We agree. We would like to investigate cases with more clients in the future work.


==> input/theory.tex <==

\newpage

\section{Potential analysis directions}

Analysis track: inspired by ensemble distillation for model fusion~\cite{lin2020ensemble}. The current FCLG can be generalized as a special case of the ensembling techniques. 

\textbf{Open Questions}
\begin{enumerate}
    \item From the domain adaptation theory~\cite{ben2010theory}, will the contrastive loss from ensembled distillation be bound by the teacher (local) models? Uniform Convergence~\cite{shalev2014understanding} may also help.
    \item Consider a simpler central model. When all the teacher models (learned from heterogeneous distributions) together with their previous rounds are available, what will be a good ensembling disillation strategy in combination of contrasting? How will the generalization/loss function change when it is changed to the 2-level contrasting? i.e. what is the trade-off?
   % \item When explaining model fusion, may Use elegant Bayesian interpretation of ensemble methods~\cite{shi2021_fed}.
\end{enumerate}

\section{Current Progress}
    \begin{enumerate}
        \item Ensemble of local model generalization bound track: Consider the simplified cases to make theoretical analysis possible. How the $L_{inter}$ can affect the generalization bound from ensemble of local models? Make the questions more approachable by the simplifying procedures: 1) Consider a binary classification task (instead of intra-contrast); 2) inter-contrast, use the representation from the final layer of the binary classifier network. 
        The generalization bound as provided by has no correlation with the distillation technique like KL-divergence~\cite{lin2020ensemble}. Not sure how to include the influence from the inter-contrast mechanism.
        \item investigate the papers which cited model contrasting (inter-contrast)~\cite{li2021_model_CFL}, currently no relevant theoretical support found.
    \end{enumerate}




\section{inter-contrast understanding for generalization bounds}

For our analysis we assume a binary classification task,
with hypothesis $h$ as a function $h: X \rightarrow  (0, 1)$.
The loss function of this binary classificatoin task is defined as $ l( \hat{y}, y) = -[y \log\hat{y} + (1 - y)\log(1-\hat{y})] $, 
where $ \hat{y} := h(x) $, is the predicted probability for the class $y = 1$.
Note that $ l(\hat{y}, y ) $ is convex with respect to $ \hat{y} $.
We denote $ \argmin_{h \in H} L_{\hat{D}} (h) $ by $ h_{\hat{D}} $.

To simplify the analysis, we consider a single example $x$ with the embedding $f(x)$ on ultimate layer of the supervised binary classification, hence $f(x)$ is two-dimension representing the probability distribution across two classes. The inter-contrast can be further described as:


\begin{align}
    \mathcal{L}_{inter}(h) &= \log \bigg (1 + \exp( f_{c}^{t}(x) \cdot f_{c}^{t-1}(x) - f_{c}^{t}(x) \cdot f_{s}(x) ) \bigg ) \nonumber \\ 
    &= \log \bigg ( \frac{\exp( f_{c}^{t}(x) \cdot f_{c}^{t-1}(x) ) + \exp( f_{c}^{t}(x) \cdot f_{s}(x) )}{\exp( f_{c}^{t}(x) \cdot f_{s}(x) )} \bigg ) \nonumber \\
    &= \log \bigg ( \frac{\exp( h_{c}^{t}(x) \cdot h_{c}^{t-1}(x) + (1-h_{c}^{t}(x)) \cdot (1-h_{c}^{t-1}(x)) ) 
    + \exp(  h_{c}^{t}(x) \cdot h_{s}(x) + (1 - h_{c}^{t}(x)) \cdot (1-h_{s}(x)) )}
    {\exp( h_{c}^{t}(x) \cdot h_{s}(x) + (1 - h_{c}^{t}(x)) \cdot (1-h_{s}(x)) )} \bigg ) \nonumber \\
    \label{eq: simple_inter}
\end{align}


\begin{enumerate}
    \item $\mathcal{L}_{inter}(h)$ can be understood as use local model representations from previous round as the negative pair samples while using the server model representations as the positive sample pairs.
    \item Alternatively, consider this as another level of supervised binary classification, use the cosine similarity between the local model and the server as the probability under true labels.
\end{enumerate}


The theorem below leverages the domain measurement tools developed in multi-domain learning theory~\cite{ben2010theory}
and provides insights for the generalization bound of the ensemble\footnote{
	The uniformly weighted hypothesis average in multi-source adaptation
	is equivalent to the ensemble of a list of models,
	by considering the output of each hypothesis/model.
} of local models (trained on local empirical distribution $\hat{D}_i$). This will only apply to the convex functions like $h(x)$ as defined before.


\begin{theorem}~\cite{lin2020ensemble}
	\label{thm:formal_risk_upper_bound_for_ensemble_model}
	Let $H$ be a hypothesis class with $\text{VCdim} (H) \leq d < \infty $.
	The difference between $ L_D ( \frac{1}{K} \sum_k h_{\hat{D}_k} ) $ and $ L_{\hat{D}} ( h_{\hat{D}} ) $,
	i.e., the distance between the risk of our ``ensembled'' model in 
	and the empirical risk of the ``virtual ERM'' with access to all local data,
	can be bounded with probability at least $ 1 - \delta $:
	\begin{small}
		\begin{align*}
			\begin{split}
				L_D \Big( \frac{1}{K} \sum_k h_{\hat{D}_k} \Big)
				&\leq
				L_{\hat{D}} ( h_{\hat{D}} )
				+ \frac{ 4 + \sqrt{ \log ( \tau_{H} (2m) ) } }{ \delta / K \sqrt{ 2m } }
				+ \frac{1}{K} \sum_{k} \left( \frac{1}{2} d_{H \Delta H} (D_k, D) + \lambda_k \right)
				\,,
			\end{split}
		\end{align*}
		where
		$ \hat{D} \!=\! \frac{1}{K} \sum_{k} \hat{D}_k $,
		$d_{H \Delta H}$ measures the domain discrepancy between two distributions~\cite{ben2010theory},
		and $\lambda_k \!=\! \inf_{h \in H} \left( L_{D} (h) \!+\! L_{D_k}(h) \right)$.
		$\tau_{H}$ is the growth function of $H$---it satisfies for all $m$, $ \tau_{H} (m) \leq \sum_{i=0}^{d} {\binom{m}{i} } $, and if $ m > d + 1 $ then $ \tau_{H} (m) \leq ( \frac{em}{d} )^{d} $.
	\end{small}
\end{theorem}


\textbf{Questions}
\begin{enumerate}
    \item How to explain Eq.\ref{eq: simple_inter} regarding different $h(x)$
    \item Can we generalize into an arbitrary feature vector, instead of probability distribution?
    \item Can we obtain a new generalization bound as affected by $L_{inter}$? i.e.how the $L_{inter}$ affects the model fusion? Understood as a regularization term? i.e regularize local representations towards their global consensus. 
\end{enumerate}


\section{Simplified model contrasting}

\subsection{central model contrasting}

Suppose we consider each isolated client as a bigger batch, within each client we will further do mini-batch training to perform intra-contrast learning. Here $l_{inter}$ consider the representations from the previous local round as negative, no matter the latent semantics. How to explain it?

\begin{algorithm}[tbh]
	\caption{FCLG simplified central train} 
	\begin{itemize}
    	\Statex{\textbf{Input}: local training epochs $E$, communication rounds $T$, number of clients $K$ and $\gamma$ the fraction of clients participating in each round.
    	}
    	\Statex{\textbf{Output}: learned model parameters $\omega^{T}$ }
	\end{itemize}
	\begin{algorithmic}[1]
	\State{initialize $\omega^{0}$}
	\For{$j = 0, 1, \cdots, T-1 $} 
            \State{Randomly sample a subset of $K_{\gamma}$ clients}
	    \For{$ i = 1, 2, \cdots, K_{\gamma}$ in parallel}
	        \State{send global model $\omega^{j}$ to $C_{i}$}
                %% start the local training part
                \State{$\omega^{0}_{i} \gets \omega^{j}$}
    \For{$t = 1, 2, \cdots, E $} 
        \For{each batch of graphs $ G_{b} \in S^{i}$}
         \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
            \State{$U^{t} \gets g(f_{\omega^{t}_{i}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}_{i}}(G_{d}) )$}
            \State{ $U_{s} \gets g(f_{\omega^{j}}(G_{b})) $; $U_{c}^{t-1} \gets g(f_{\omega_{i}^{t-1}}(G_{b})) $}
            \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} and $l_{inter}$ from Eq.\ref{eq: graph-level CL server and client}}
            \State{$l_{tot} \gets l_{inter} +  l_{intra} $ }  % 
            \State{SGD update on $\omega^{t}_{i}$}
    	\EndFor
	\EndFor
        \State{$\omega_{i}^{j} \gets \omega^{E}_{i}$}
            %% End of the local train
	    \EndFor
	    \State{$\omega^{j+1} \gets \sum^{K_{\gamma}}_{i}\frac{|S^{i}|}{|S|}\omega^{j}_{i}$}
	\EndFor
	%% =============Sever above =================
	\end{algorithmic} 
\end{algorithm}


\subsection{FL ensembling distillation with using server data}

Consider there are extra data on the server to test/correct the generalization performance as used by~\cite{chen_2020_fedbe}. Any insights or potential connections?

\begin{algorithm}[tbh]
	\caption{FL ensembling with separate data on the server~\cite{chen_2020_fedbe}} 
	\label{alg:FCLG server data}
	\begin{itemize}
    	\Statex{\textbf{Input}: local training epochs $E$, communication rounds $T$, number of clients $K$
    	}
    	\Statex{\textbf{Output}: learned model parameters $\omega^{T}$ }
	\end{itemize}
	\begin{algorithmic}[1]
	\State{\textbf{Server:}}
	\State{initialize $\omega^{0}$}
	\For{$j = 0, 1, \cdots, T-1 $} 
	    \For{$ i = 1, 2, \cdots, K$ in parallel}
	        \State{send global model $\omega^{j}$ to $C_{i}$}
	        \State{$\omega_{i}^{j} \gets $ \textbf{Client($i, \omega^{j}$)}}
	    \EndFor
	    \State{$\omega^{j+1} \gets \sum^{K}_{i}\frac{|S^{i}|}{|S|}\omega^{j}_{i}$}
        \For{each batch of graphs $ G_{b} \in S_{0}$}
         \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
            \State{$U^{t} \gets g(f_{\omega^{t}_{i}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}_{i}}(G_{d}) )$}
            \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} }
            \State{SGD update on $\omega^{t}_{i}$}
    	\EndFor
	\EndFor
	\State{return $\omega^{T}$}
	%% =============Sever above =================
	\State{\textbf{Client($i, \omega^{j}$):}}
    \State{$\omega^{0}_{i} \gets \omega^{j}$}
    \For{$t = 1, 2, \cdots, E $} 
        \For{each batch of graphs $ G_{b} \in S^{i}$}
         \State{$G_{d} \gets $ graph diffusion on $G_{b}$}
            \State{$U^{t} \gets g(f_{\omega^{t}_{i}}(G_{b}))$; $V^{t} \gets g( f_{\omega^{t}_{i}}(G_{d}) )$}
            \State{Calculate $l_{intra} $ from Eq.\ref{eq:CL_loss} }
            \State{SGD update on $\omega^{t}_{i}$}
    	\EndFor
	\EndFor
	\State{return $\omega^{E}_{i}, U^{E}_{i}$ }
	\end{algorithmic} 
\end{algorithm}  




